CineMPC: Controlling Camera Intrinsics and Extrinsics for Autonomous Cinematography

We present CineMPC, an algorithm to autonomously control a UAV-borne video camera in a nonlinear Model Predicted Control (MPC) loop. CineMPC controls both the position and orientation of the camera -- the camera extrinsics -- as well as the lens focal length, focal distance, and aperture -- the camera intrinsics. While some existing solutions autonomously control the position and orientation of the camera, no existing solutions also control the intrinsic parameters, which are essential tools for rich cinematographic expression. The intrinsic parameters control the parts of the scene that are focused or blurred, the viewers' perception of depth in the scene and the position of the targets in the image. CineMPC closes the loop from camera images to UAV trajectory and lens parameters in order to follow the desired relative trajectory and image composition as the targets move through the scene. Experiments using a photo-realistic environment demonstrate the capabilities of the proposed control framework to successfully achieve a full array of cinematographic effects not possible without full camera control.

==> 99_Implementation.tex <==
\begin{figure*}[!th]
     \includegraphics[width=\linewidth]{images/architecture_graph/cineMPC_graph.JPG}
	\caption{\footnotesize CineMPC graph}
	\label{fig:parameters}
\end{figure*}
The implementation of the platform is composed by different modules. These modules and their communications are represented in \ref{fig:parameters}. Although this graph represents a generic version of the platform, in this section we will explain how we have implemented the solution following this pattern.

\subsection{Coordinator}
This module is the core of the system. It takes care of all the communications between the different modules, as well as to provide the necessary elements to the MPC problem to solve the problem.
%In our solution, the whole system is implemented in C++. 

\subsection{User}
The user specifies the constraints of the MPC problem, $\mathbf{J^*}$, and the set of weights,  $\mathbf{w}$, according to their artistic objectives. $\mathbf{J^*}$ will be composed of each one of the cost terms elements that are explained in \red{ref sec 3} section III, $\mathbf{J^*} = \lbrace{D_{n}}^{*},\ D_{f}^{*},\ \textit{im}^{*},\ d^{*},\ ^{d}R_{s}^{*}\rbrace $ as well as  $\mathbf{w}$ represents the set of weights of the cost function $\mathbf{w} = \lbrace{w_{D_{n}}},\ w_{D_{f}},\ w_{im_t},\ w_{d_t},\ w_{R_t}\rbrace $.

\subsection{Scene}
The scene is the representation of the world where all the elements, including the recording drone, are placed. The scene will contain the $n$ targets we want to record.
%Our representation of the world and the scene are done with Unreal Engine 4 \cite{unreal}. 


\subsection{Drone}
The drone will be equipped with a RGB-D camera in the way it can extract the RGB image and the depth map for further processing. Moreover, we will assume that it accounts with a low level controller that will take actions to its actuators in terms of the given instructions.
 MPC will give the controller a trajectory of $N$ 3D points that artistically improve the footage. For the optimization of the trajectory we can use one of the existing trajectory planners, like the one presented in \cite{richter2016polynomial}. The input of this approach is a set of waypoints where we want the drone to pass through. In our system, this points are given by MPC. The output   that follows some time and soften restrictions and can be introduced to the low level controller to the drone to execute the actions.
% For our implementation, we have used CinemAirSim, a photorealistic robotics simulator for cinematographic purposes \cite{pueyo2020cinemairsim}. It enlarges AirSim, the robotic simulator of \cite{shah2018airsim}, with a realistic configurable cinematographic cameras that implements the pin-hole model. AirSim implements a low-level controller for the drone that takes a trajectory of 3D world points and a desired velocity as an input and moves the drone accordingly.
% Moreover, AirSim provides the depth map from the drone perspective as well as the RGB image.

\subsection{Perception}
For the localization of the targets in the scene our system will have a perception module. This module receives the RGB image and the depth map as an input. Then it localizes the targets in the RGB image and provides the position of the targets in the image, expressed in pixels. Afterward, thanks to the depth map, by using some geometric transformations, this position in the image is transformed in world coordinates, in meters. The output of this module will express the relative position of the targets with respect to the camera in 3D coordinates, $\mathbf{x}_{t,k}^{\lbrace i:n\rbrace}$.
% In our solution, we use Yolov4 (~\cite{bochkovskiy2020yolov4}) to get the bounding boxes of the targets of the image. Then, thanks to the depth map obtained from AirSim, we can obtain the state of the targets with respect to the drone as previously described.

\subsection{MPC}
MPC calculates the values of the control parameters for the present time $k$ to the to the $k+N$ time steps. In this way, it can optimize the current state of the system to minimize the value of a cost function and take actions with the actuators accordingly. In our system, the set of parameters that MPC receives at the time step $k$ are: the drone state, $\mathbf{x}_{d,k}$, the state of the $n$ targets, $\mathbf{x}_{t,k}^{i:n}$, the camera state, $\mathbf{\sigma}_k$ and the set of cost terms, $\mathbf{J*}$, and weighs, $\mathbf(w)$ that the user gives.
Thanks to an optimization library, it calculates the present and future $k:k+N$ time steps of the state of the drone, $\mathbf{x}_{d,k:k+N}$, and the state of the camera $\mathbf{\sigma}_{k:N}$ in which the cost will be reduced. Then, it gives these new values to the coordinator to take actions.

% As this problem is a non-linear, we needed a non-linear optimization library to be the core of our MPC module. We have used Ipopt (Interior Point OPTimizer) \cite{wachter2006implementation} in our implementation.
\subsection{Depth of Field}
This module will communicate with the MPC module. MPC gives this module some of the intrinsic parameters of the lens of the camera($F_{k:k+N}, f_{k:k+N}, A_{k:k+N}$), in the instant $k$ and in the $N$ next steps and this module will provide the near and far distances ($D_{n_{k:k+N}}, D_{f_{k:k+N}}$), limits of the depth of field for each of these present and future steps. 
\subsection{Image Position}
MPC will provide this module with the relative distance and rotation drone-targets, $\mathbf{^{d}P_{t}}_{k:k+N}^{i:n}$ and $\mathbf{^{d}R_{t}}_{k:k+N}^{i:n}$, as well as some of the intrinsic parameters of the camera: the focal length, $f_{k:k+N}$, and the ratio $\beta$, that relates the size of the sensor in millimeters with the size of the image that the sensor produces, in pixels.
By using all these information, the image position module module implements some geometrical transformations to provide the MPC the position in the image of the targets for the present step $k$ and the $N$ following steps, $\mathbf{im}^{i:n}_{k:k+N}$.
